Contextual Representation Learning beyond Masked Language Modeling

How do masked language models (MLMs) such as BERT learn contextual representations? In this work, we analyze the learning dynamics of MLMs. We find that MLMs adopt sampled embeddings as anchors to estimate and inject contextual semantics to representations, which limits the efficiency and effectiveness of MLMs. To address these issues, we propose TACO, a simple yet effective representation learning approach to directly model global semantics. TACO extracts and aligns contextual semantics hidden in contextualized representations to encourage models to attend global semantics when generating contextualized representations. Experiments on the GLUE benchmark show that TACO achieves up to 5x speedup and up to 1.2 points average improvement over existing MLMs. The code is available at https://github.com/FUZHIYI/TACO.

==> 010intro.tex <==

Learning good representations for text is a fundamental problem in natural language processing. In the era of deep learning, language representation learning mainly studies the distributional semantics, which defines semantic similarity in terms of vector similarity. With the availability of large-scale raw data, language modeling (LM), a self-supervised task, has been the dominant choice for representation learning. 
And in recent years, the pre-trained LMs with contextual representation have achieved promising performance on various downstream NLP tasks~\citep{DBLP:conf/naacl/PetersNIGCLZ18,DBLP:conf/naacl/DevlinCLT19,DBLP:journals/jmlr/RaffelSRLNMZLL20,DBLP:conf/nips/BrownMRSKDNSSAA20}. 

Conventional approaches~\citep{DBLP:conf/nips/MikolovSCCD13,DBLP:conf/emnlp/PenningtonSM14} (e.g., Word2Vec) exploit Harris's hypothesis ---
words that occur in the same contexts tend to have similar meanings~\citep{harris1954distributional}. 
Therefore, tokens (or words) with similar contexts may lead to close embeddings in a neural model. 
However, recent pre-trained language models such as BERT~\citep{DBLP:conf/naacl/DevlinCLT19} and  GPT3~\citep{DBLP:conf/nips/BrownMRSKDNSSAA20} actually do not explicitly model this hypothesis. Instead, they implement various contextual representation learning objectives. 
They either use next token prediction or masked token prediction as the training objective, where the context is either left prefix or surrounding text. 
We argue that the current objectives of token prediction, whether masked or not, may not be adequate, which is also verified by our experiments and several recent studies~\citep{DBLP:journals/corr/abs-1911-05758,DBLP:conf/emnlp/VulicPLGK20,aless2021comprehensive}. 

In this paper, we study training objectives for language representation learning. 
Inspired by Harris's hypothesis, we propose three hypotheses for a good language representation space. 
In nowadays LMs, a token is associated with two types of representations: a context-independent representation (i.e., embedding) and multiple context-dependent (or contextualized) representations. 
That is consistent with the theory of concepts by \citet{Barsalou1982ContextindependentAC}.
However, what is the relation between context-independent and context-dependent representations?
There can be three relations concerning the representation of tokens, including relations among
\begin{inparaenum}[\it a)]
\item \emph{different} context-independent representations,
\item context-independent and context-dependent representations for the \emph{same} token,
\item context-dependent representations for \emph{different} tokens with the \emph{same} context or across \emph{different} contexts. 
\end{inparaenum}
We propose the following three hypotheses (referred to as DPH hypotheses) concerning these three relations. 
\begin{itemize*}
    \item[H1] \textbf{Distinguishable}: different tokens should have distinct context-independent representations; 
    \item[H2] \textbf{Proximal}: a token should have context-dependent representations similar to its context-independent representation and dissimilar to other tokens' context-independent representations;
    \item[H3] \textbf{Homophily}: tokens in the same context should have similar contextualized representation. 
\end{itemize*}

According to these three hypotheses, we analyze the prevalent masked language modeling (MLM) objective.  MLM can satisfy the first two hypotheses relatively easily while struggling to capture the Homophily hypothesis.  Intuitively,  MLM aims to draw context-dependent representation closer to its context-independent representation for masked tokens. Only when the masked tokens have similar context-independent representations can the Homophily hypothesis be achieved. Therefore, MLM is low efficiency on modeling the Homophily hypothesis. Motivated by this investigation, we propose a novel self-supervised objective, \textbf{T}oken-level \textbf{C}ontrastive (\objective) loss,  for training contextual language representations. It explicitly encourages context-dependent representations for different tokens under similar contexts to stay close to each other (H3). By combining \objective with MLM, we can train a \textbf{T}oken contr\textbf{A}stive \textbf{CO}ntextualized representation model, \method, which simultaneously maintains the three objectives from the DPH hypotheses. 

The contributions of this paper are as follows.
\begin{itemize*}
    \item We propose DPH hypotheses to guide language representation learning; 
    \item We propose a simple yet efficient method \method to implement these hypotheses for contextual representation learning; 
    \item Our experiments show that \method outperforms existing language representation baselines with up to 1.3 point improvement while achieves up to 5x speedup to obtain the same performance with baselines on GLUE benchmark. 
\end{itemize*}

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{fig/approach_newest.pdf}
    \caption{An illustration of the DPH hypotheses. The Distinguishable hypothesis and the Proximal hypothesis ensure a token is identifiable given its contextualized representation. The Homophily hypothesis requires the contextualized representation of tokens in the same context to be similar. Therefore, the DPH hypotheses can recover the distributional hypothesis in the context of contextual language representation learning. }
    \label{fig:framework}
\end{figure}

